Operating data of a specific Aquatic Center as a Benchmark for dynamic model learning: search for a valid prediction model over an 8-hour horizon

This article presents an identification benchmark based on data from a public swimming pool in operation. Such a system is both a complex process and easily understandable by all with regard to the stakes. Ultimately, the objective is to reduce the energy bill while maintaining the level of quality of service. This objective is general in scope and is not limited to public swimming pools. This can be done effectively through what is known as economic predictive control. This type of advanced control is based on a process model. It is the aim of this article and the considered benchmark to show that such a dynamic model can be obtained from operating data. For this, operational data is formatted and shared, and model quality indicators are proposed. On this basis, the first identification results illustrate the results obtained by a linear multivariable model on the one hand, and by a neural dynamic model on the other hand. The benchmark calls for other proposals and results from control and data scientists for comparison.

==> a.tex <==

\section{Evaluation de la qualité des deux modèles proposés}

\paragraph{\textbf{State space estimation }} We use a linear state space model with a subspace identification method \cite{ljung1998system}. This identification is performed with the Matlab tools box \cite{matlabid} (\textit{ssest} function). This method uses all inputs signals mentioned earlier. 
\begin{equation}
\begin{gathered}
    x[k+1] = A x[k] + B u[k] \\
    y[k]   = C x[k]
\end{gathered}
\end{equation}

To perform prediction, we use the function \textit{forecast} which perform an ordinary least square method to estimate the initial state with respect to the size of the given past horizon.  

\paragraph{\textbf{NLARX estimation}} For the nonlinear part, we use a neural network in a NLARX formulation. 

\begin{equation}
    y[k+1] = f_{\theta} (y[k], \cdots y[k-n_a], u[k],  \cdots, u[k-n_b])
\end{equation}

This model is coupled with a MPC relevant identification loss function with the BPTT (Back Propagation Through Time) \cite{Werbos1990} method and Tensorflow library \cite{tensorflow2015-whitepaper}. The loss function can be describe with the following formula.
\begin{equation}
    \mathcal{L}(\theta) = \frac{1}{N}\sum_{n=0}^{N-1} \frac{1}{P}\sum_{p=0}^{P-1} \left( \hat{y}(t_0(n)+p | t_0(n), \theta ) - y(t_0(n)+p) \right)^2
\end{equation}

With $\hat{y}(t_0(n)+p | t_0(n), \theta )$, the model prediction given the state at $t_0(n)$ and the exogenous data from $t_0(n)+p $ to $t_0(n)$. The prediction is done like the full future prediction in \cite{MENDOZASERRANO20141301}. We use the solver ADAM \cite{kingma2014method} a unconstrained non linear solver.



The forecast is performed in iterative way like its describe here \cite{} \todo{ref}. We choose to stay with a one step ahead prediction instead of another formulation to force an interpretable dynamic model.

We trained both linear and non linear models with the same MIMO formulation and procedure. An hyper optimisation procedure was used using a cross validation method to reduce bias with this relatively small dataset.
The cross validation is done with data sections instead of regression entry to avoid overlap between samples.
The testing dataset is placed in the dataset extremum to avoid any data leak.  All the optimized parameters are details table \ref{tab:opti_nlarx_param} and \ref{tab:opti_ss_param}. 

\vspace{5pt}


\begin{table}
\centering
\begin{tabular}{|c | c|}
\hline
 Parameters & Values \\
\hline
 N\# layers & \{1,2,3\}  \\
  N\# unit per layer & \{8,16,32,64\}  \\
  learning rate  & [1e-5, 1e-2]  \\
  batch size  & [16,256] \\
  l2 penalization & \{0.0,1e-4,1e-3\} \\
  loss function horizon & [3, 5, 8, 15] \\
\hline
\end{tabular}
\caption{optimized NLARX model's parameters}
\label{tab:opti_nlarx_param}
\end{table}
\begin{table}
\centering
\begin{tabular}{|c|c|}
\hline
 Parameters & Values \\
\hline 
 $n_x$ & [2, 3, 4]  \\
 focus & simulation, prediction  \\
 subspace horizon & \{48, 24, -1\}  \\
 noise model & \{None, Estimate\} \\
 \hline
\end{tabular}
\caption{optimized SS model's parameters}
\label{tab:opti_ss_param}

\end{table}

\subsection{Performance and limits}

We first introduce the raw prediction accuracy of the two selected model. We plo the accuracy with respect to the prediction depth (like \cite{Gopaluni2004,Thilker2022}). The RMSE  and R$^2$ are available figure \ref{fig:rmse_model} and \ref{fig:r2_model}. It was computed with test part of the dataset. The model is train with the optimal parameters obtain in the optimization. 

\begin{figure}
  \centering
  \includegraphics[width=0.8\linewidth]{./image/rmse_acc.pdf}
  \caption{RMSE accuracy according to prediction depth.}
  \label{fig:rmse_model}
\end{figure}%
\begin{figure}
  \centering
  \includegraphics[width=.8\linewidth]{./image/r2_acc.pdf}
  \caption{R$^2$ accuracy according to prediction depth.}
      \label{fig:r2_model}
\end{figure}

As expected, the accuracy decreases according to the prediction dept. The neural network model achieve a higher accuracy than the linear one. This gap is more pronounce with the second pool which is more difficult to predict with higher temperature and people activity more intense.  We can achieve for the NLARX model a R$^2$ score above 0.85 during the whole 8 hours horizons. \todo{rajouter un comparatif ? }



The figure \ref{fig:pred_temporal} display the prediction of both model for every batch of 8 hours. The prediction only uses exogenous data to achieve the multi one step ahead prediction. 


\begin{figure}[ht]
    \centering
    \caption{Prediction on testing data }
    \label{fig:pred_temporal}
\end{figure}

We can now try these models with the extrapolation data. The scenarios used were collected with the same system but in non nominal situation. We use them to show the extrapolation result of our model with the real system. This extrapolation data is not used for training.
As described in the section \ref{seq:system_id}, our first scenario is a large decrease of temperature. We show in figure \ref{fig:extrapol} this scenario with both models prediction.


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{./image/extrapol.pdf}
    \caption{Prediction with NLARX model and extrapolation data }
    \label{fig:extrapol}
\end{figure}

\todo[inline]{Rajouter modèle linéaire}

The linear model thank's to its horizon and its stable pole position, perfleeclty predict the temp... A FINIR 
Other data extrapolation result are available at appendix \ref{ap:result_extra}



%Faire le tableau pour récapituler les perforamcen et les emttre en perspective


Finally, we want to show the possibility of using models as is in a EMPC context. Therefore, we put our model to a EMPC formulation with the pool requirements to obtain the potential temperature scheduling that can be produced with a purely data driven model (controller formulation is available at append \ref{ap:empc}). 




Both figure \ref{fig:arx_EMPC_1a} and \ref{fig:arx_EMPC_2} compare the EMPC planning with the real data. We can first see the same idea to reduce the temperature and increase it again just before the pool opens. We have to cite this behaviour since the model is pure black box model that do not necessary perfectly understood the energy loss dynamic. The major difference here is the heating time to achieve the target temperature. This duration depends on other exogenous data not present  here to add enough insight to perfectly predict this heating time. This can be due to a lack of information or poor training process. A  forgetting coefficient can be added to the continuous training of this approach but we will not detail it here.


Nevertheless, this model provides compliant results according to what was expected. This first result motivates experimentation with this back box formulation to see the closed loop behaviour between the implicit controller, the model and the system. 
